Multi-Instance Pose Networks: Rethinking Top-Down Pose Estimation

A key assumption of top-down human pose estimation approaches is their expectation of having a single person/instance present in the input bounding box. This often leads to failures in crowded scenes with occlusions. We propose a novel solution to overcome the limitations of this fundamental assumption. Our Multi-Instance Pose Network (MIPNet) allows for predicting multiple 2D pose instances within a given bounding box. We introduce a Multi-Instance Modulation Block (MIMB) that can adaptively modulate channel-wise feature responses for each instance and is parameter efficient. We demonstrate the efficacy of our approach by evaluating on COCO, CrowdPose, and OCHuman datasets. Specifically, we achieve 70.0 AP on CrowdPose and 42.5 AP on OCHuman test sets, a significant improvement of 2.4 AP and 6.5 AP over the prior art, respectively. When using ground truth bounding boxes for inference, MIPNet achieves an improvement of 0.7 AP on COCO, 0.9 AP on CrowdPose, and 9.1 AP on OCHuman validation sets compared to HRNet. Interestingly, when fewer, high confidence bounding boxes are used, HRNet's performance degrades (by 5 AP) on OCHuman, whereas MIPNet maintains a relatively stable performance (drop of 1 AP) for the same inputs.

==> prev_cvpr_tables_rebuttal/resnet101.tex <==
\begin{table}[b]
\captionsetup{font=small}
  \vspace*{-0.15in}
    \resizebox{3.3in}{!}{
    \setlength{\tabcolsep}{1.5pt}
    \renewcommand{\arraystretch}{1.0} % Default value: 1
    \begin{tabular}{@{}l|c c c| c c c| c c c@{}}
    \hline
   \multirow{2}{*}{Method} & \multicolumn{3}{c|}{COCO} & \multicolumn{3}{c|}{CrowdPose} & \multicolumn{3}{c}{OCHuman}\\
    & $\text{AP}$ & $\text{AP}^{50}$ & $\text{AP}^{75}$ & $\text{AP}$ & $\text{AP}^{50}$ & $\text{AP}^{75}$ & $\text{AP}$ & $\text{AP}^{50}$ & $\text{AP}^{75}$ \\
    \hline
    CSM+SCARB [2] & 73.8 &  91.7 & 81.4 & - &  - & - & - & - & - \\
    MDN [4] & 52.3 &  77.2 & 58.0 & - &  - & - & - & - & - \\
    MaskRCNN & 64.8 &  - & - & 57.2 &  83.5 & 60.3 & 20.2 & 33.2 & 24.5 \\
    SBL & 73.7 &  91.9 & 81.8 &60.8 &  81.4 & 65.7 & 24.1 & 37.4 & 26.8 \\
    AlphaPose   & 70.1 &  - & - & 61.0 &  81.3 & 66.0 & - &  - & - \\
    CrowdPose[5] & 70.9 &  - & - & 66.0 &  81.4 & 65.7 & - &  - & - \\
    AlphaPose+  & 72.2 &  90.1 & 79.3  & 68.5 &  86.7 & 73.2 & 27.5 & 40.8 & 29.9 \\
    OPEC-Net[6] & 73.9 &  91.9 & \textbf{82.2}  & \textbf{70.6} &  \textbf{86.8} & \textbf{75.6} & 29.1 &  41.3 & 31.4\\
    MHPNet (Ours) & \textbf{74.2} &  \textbf{92.4} & 81.9 & 68.1 & 86.3 & 73.4 & \textbf{40.0} & \textbf{51.0} & \textbf{44.0} \\
    \hline
    \end{tabular}
    }
    \vspace*{-0.1in}
    \caption{All methods use ResNet-101 backbone (except MDN) and YOLO-v3 detector (except CSM+SCARB and MDN).}
    \label{tab:resnet101}
    \vspace*{-0.2in}
\end{table}

==> prev_cvpr_tables_rebuttal/single_multi.tex <==
% \begin{table}[b]
% % \captionsetup{font=scriptsize}
% \captionsetup{font=small}
% %   \vspace*{-0.15in}
%     % \setlength{\tabcolsep}{1.5pt}
%     \small
%     \renewcommand{\arraystretch}{1.0} % Default value: 1
%     \begin{tabular}{@{}l|c c c|c c c}
%     \hline
%   \multirow{2}{*}{Method} & \multicolumn{3}{c|}{COCO} & \multicolumn{3}{c}{OCHuman}\\
%     & $\text{AP}$ & $\text{AP}^{50}$ & $\text{AP}^{75}$ & $\text{AP}$ & $\text{AP}^{50}$ & $\text{AP}^{75}$  \\
%     \hline
%     HRNet & 75.5 & 92.5 & 83.3 & 37.2 & 46.7 & 40.0\\
%     HRNet* & \textbf{75.8} & \textbf{92.8} & \textbf{83.6} & 37.8 & 46.9 & 41.2\\
%     MHPNet & 75.3 & 92.1 & 83.0 & \textbf{42.5} & \textbf{51.8} & \textbf{46.3}\\
%     \hline
%     \end{tabular}
%     \vspace*{-0.1in}
%     \caption{Comparison of HRNet (single-scale, 1 inference), HRNet* (six-scale, 6 inferences) and MHPNet (single-scale, 2 inferences) on \texttt{test} sets using HRNet-48-384 backbone and Faster-RCNN.}
%     \label{tab:single_multi}
%     \vspace*{-0.2in}
% \end{table}

\begin{table}[b]
% \captionsetup{font=scriptsize}
\captionsetup{font=small}
  \vspace*{-0.2in}
    \resizebox{2.9in}{!}{
    \setlength{\tabcolsep}{1.9pt}
    \small
    \renewcommand{\arraystretch}{1.0} % Default value: 1
    \begin{tabular}{@{}l|c c c|c c c|c c c}
    \hline
   \multirow{2}{*}{Method} & \multicolumn{3}{c|}{COCO} & \multicolumn{3}{c|}{OCHuman} & \multicolumn{3}{c}{OCPose [6]}\\
    & $\text{AP}$ & $\text{AP}^{50}$ & $\text{AP}^{75}$ & $\text{AP}$ & $\text{AP}^{50}$ & $\text{AP}^{75}$ & $\text{AP}$ & $\text{AP}^{50}$ & $\text{AP}^{75}$  \\
    \hline
    HRNet & 75.5 & 92.5 & 83.3 & 37.2 & 46.7 & 40.0 & 30.2 & 48.3 & 23.1\\
    HRNet* & \textbf{75.8} & \textbf{92.8} & \textbf{83.6} & 37.8 & 46.9 & 41.2 & 31.1 & 49.1 & 24.7\\
    MHPNet & 75.3 & 92.1 & 83.0 & \textbf{42.5} & \textbf{51.8} & \textbf{46.3} & \textbf{39.2} & \textbf{61.2} & \textbf{32.6}\\
    \hline
    \end{tabular}
    }
    \vspace*{-0.1in}
    \caption{Comparison of HRNet (single-scale, 1 inference), HRNet* (six-scale, 6 inferences) and MHPNet (single-scale, 2 inferences) on \texttt{test} sets using HRNet-48-384 backbone and Faster-RCNN.}
    \label{tab:single_multi}
    \vspace*{-0.2in}
\end{table}

==> sections/experiments/ocpose.tex <==
\textbf{Dataset:} OCPose is a larger dataset with pose annotations of occluded humans. It contains $9K$ images and $18000$ persons labeled with $12$ keypoints. The number of examples with occlusion IoU $>0.5$ is $78\%$ for OCPose~\cite{qiu2020peeking}.

\textbf{Results:} \rawal{work in progress, the annotations are corrupted, trying to fix}

==> tables/resnet101.tex <==
\begin{table}[b]
\captionsetup{font=small}
  \vspace*{-0.15in}
    \resizebox{3.3in}{!}{
    \setlength{\tabcolsep}{1.5pt}
    \renewcommand{\arraystretch}{1.0} % Default value: 1
    \begin{tabular}{@{}l|c c c| c c c| c c c@{}}
    \hline
   \multirow{2}{*}{Method} & \multicolumn{3}{c|}{COCO} & \multicolumn{3}{c|}{CrowdPose} & \multicolumn{3}{c}{OCHuman}\\
    & $\text{AP}$ & $\text{AP}^{50}$ & $\text{AP}^{75}$ & $\text{AP}$ & $\text{AP}^{50}$ & $\text{AP}^{75}$ & $\text{AP}$ & $\text{AP}^{50}$ & $\text{AP}^{75}$ \\
    \hline
    CSM+SCARB [2] & 73.8 &  91.7 & 81.4 & - &  - & - & - & - & - \\
    MDN [4] & 52.3 &  77.2 & 58.0 & - &  - & - & - & - & - \\
    MaskRCNN & 64.8 &  - & - & 57.2 &  83.5 & 60.3 & 20.2 & 33.2 & 24.5 \\
    SBL & 73.7 &  91.9 & 81.8 &60.8 &  81.4 & 65.7 & 24.1 & 37.4 & 26.8 \\
    AlphaPose   & 70.1 &  - & - & 61.0 &  81.3 & 66.0 & - &  - & - \\
    CrowdPose[5] & 70.9 &  - & - & 66.0 &  81.4 & 65.7 & - &  - & - \\
    AlphaPose+  & 72.2 &  90.1 & 79.3  & 68.5 &  86.7 & 73.2 & 27.5 & 40.8 & 29.9 \\
    OPEC-Net[6] & 73.9 &  91.9 & \textbf{82.2}  & \textbf{70.6} &  \textbf{86.8} & \textbf{75.6} & 29.1 &  41.3 & 31.4\\
    MIPNet (Ours) & \textbf{74.2} &  \textbf{92.4} & 81.9 & 68.1 & 86.3 & 73.4 & \textbf{40.0} & \textbf{51.0} & \textbf{44.0} \\
    \hline
    \end{tabular}
    }
    \vspace*{-0.1in}
    \caption{For a fair comparison, all methods use ResNet-101 backbone (except MDN) and YOLO-v3 detector (except CSM+SCARB and MDN).}
    \label{tab:resnet101}
    \vspace*{-0.2in}
\end{table}

==> tables_rebuttal/modulation_variants.tex <==
% \begin{table}[b]
\begin{table}
\centering
% \captionsetup{font=scriptsize}
\captionsetup{font=small}
%   \vspace*{-0.2in}
    \setlength{\tabcolsep}{1.9pt}
    \small
    \renewcommand{\arraystretch}{1.0} % Default value: 1
    \begin{tabular}{@{}l|c c c|c c c@{}}
    \hline
   \multirow{2}{*}{Modulation Variant ($\mathbf{m}$)} & \multicolumn{3}{c|}{COCO} & \multicolumn{3}{c}{OCHuman}\\
    & $\text{AP}$ & $\text{AP}^{50}$ & $\text{AP}^{75}$ & $\text{AP}$ & $\text{AP}^{50}$ & $\text{AP}^{75}$   \\
    \hline
    $\mathbf{F}_{ex}(\mathbf{s} \oplus \boldsymbol{\lambda})$  & 74.7 & 91.8 & 80.2 & 61.8 & 79.8 & 68.4 \\
    $\mathbf{F}_{ex}(\mathbf{s} * \mathbf{F}_{em}(\boldsymbol{\lambda}))$ & 77.2 & 94.4 & 84.7 & 71.1 & 87.5 & 77.8 \\
     $\mathbf{F}_{ex}(\mathbf{s})*\mathbf{F}_{em}(\boldsymbol{\lambda})$ (Ours) & \textbf{77.6} & \textbf{94.4} & \textbf{85.3} & \textbf{72.5} & \textbf{89.2} & \textbf{79.4} \\
    \hline
    \end{tabular}

    \vspace*{-0.1in}
    \caption{Comparison of MIMB (Ours) with different instance modulation variants using HRNet-W32 backbone with $256 \times 192$ input resolution and ground-truth bounding boxes on the \texttt{val} sets.}
    \label{tab:modulation}
    \vspace*{-0.25in}
\end{table}

==> tables_rebuttal/multiple_averaged_runs.tex <==


% \begin{table}[b]
\begin{table}[b]
\centering
\captionsetup{font=small}
  \vspace*{-0.2in}
    \resizebox{3.3in}{!}{
    \small
    \renewcommand{\arraystretch}{1.0} % Default value: 1
  \begin{tabular}{@{}l|l|l|l|l@{}}
    \hline
Method  & Arch & $\text{AP}$ & $\text{AP}^{50}$ & $\text{AP}^{75}$   \\
    \hline
    
    HRNet  & H-32 & $76.5$ & $93.5$ & $83.7$ \\
    MIPNet & H-32 & $\mathbf{77.44 \pm 0.185}$ & $\mathbf{94.42 \pm 0.039}$ & $\mathbf{85.32\pm 0.025}$  \\
    
    \hline
    
    HRNet & H-48 & 77.1 & 93.6 & 84.7\\
    MIPNet & H-48 & $\mathbf{77.84 \pm 0.162}$ & $\mathbf{94.44 \pm 0.079}$ & $\mathbf{85.4\pm 0.012}$ \\
    
    \hline

    \end{tabular}
    }
    \vspace*{-0.1in}
    \caption{We report mean $\pm$ std-dev of MIPNet over five runs on the COCO \texttt{val} set with ground-truth bounding boxes using $256 \times 192$ input resolution. H-@ stands for HRNet-W@ backbone.}
    \label{tab:averaged_runs}
    \vspace*{-0.2in}
\end{table}

% % \begin{table}[b]
% \begin{table}[b]
% \centering
% \captionsetup{font=small}
%   \vspace*{-0.2in}

%     \small

%   \begin{tabular}{@{}l|l|l|l|l@{}}
%     \hline
% Method  & Arch & $\text{AP}$ & $\text{AP}^{50}$ & $\text{AP}^{75}$   \\
%     \hline
    
%     HRNet  & H-32 & $76.5$ & $93.5$ & $83.7$ \\
%     MIPNet & H-32 & \scriptsize{$\mathbf{77.44 \pm 0.185}$} & \scriptsize{$\mathbf{94.42 \pm 0.039}$} & \scriptsize{$\mathbf{85.32\pm 0.025}$} \\
    
%     \hline
    
%     HRNet & H-48 & 77.1 & 93.6 & 84.7\\
%     MIPNet & H-48 & \scriptsize{$\mathbf{77.84 \pm 0.162}$} & \scriptsize{$\mathbf{94.44 \pm 0.079}$} & \scriptsize{$\mathbf{85.4\pm 0.012}$} \\
    
%     \hline

%     \end{tabular}

%     \vspace*{-0.1in}
%     \caption{We report the mean and std-dev of MIPNet over five independent runs on the COCO \texttt{val} set with ground-truth bounding boxes using $256 \times 192$ input resolution. H-@ stands for HRNet-W@ backbone.}
%     \label{tab:averaged_runs}
%     \vspace*{-0.2in}
% \end{table}

==> tables_rebuttal/two_head_baseline.tex <==
% \begin{table}[b]
\begin{table}[b]
\centering
% \captionsetup{font=scriptsize}
\captionsetup{font=small}
  \vspace*{-0.2in}
    \setlength{\tabcolsep}{1.9pt}
    \small
    \renewcommand{\arraystretch}{1.0} % Default value: 1
    \begin{tabular}{@{}l|c|c c c|c c c@{}}
    \hline
   \multirow{2}{*}{Method} & \multirow{2}{*}{\#Params} & \multicolumn{3}{c|}{COCO} & \multicolumn{3}{c}{OCHuman}\\
    & & $\text{AP}$ & $\text{AP}^{50}$ & $\text{AP}^{75}$ & $\text{AP}$ & $\text{AP}^{50}$ & $\text{AP}^{75}$   \\
    \hline
    HRNet & 28.5M & 76.5 & 93.5 & 83.7 & 63.1 & 79.4 & 69.0 \\
    Two-Heads (\textit{light}) & 28.6M & 76.7 & 93.4 & 84.0 & 64.0 & 78.7 & 71.2 \\
    Two-Heads (\textit{heavy}) & 48.9M & 77.1 & 94.1 & \textbf{85.5} & 69.8 & 84.5 & 74.9 \\
    MIPNet & 28.6M & \textbf{77.6} & \textbf{94.4} & 85.3 & \textbf{72.5} & \textbf{89.2} & \textbf{79.4} \\
    \hline
    \end{tabular}

    \vspace*{-0.1in}
    \caption{Comparison of MIPNet with the Two-Heads baseline (\textit{light}, \textit{heavy}) and HRNet on the \texttt{val} sets using HRNet-W32 backbone with $256\times192$ input resolution and ground-truth bounding boxes.}
    \label{tab:two_head_baseline}
    % \vspace*{-0.2in}
\end{table}
